Large Language Models for Business Process Management: Opportunities and Challenges

Large language models are deep learning models with a large number of parameters. The models made noticeable progress on a large number of tasks, and as a consequence allowing them to serve as valuable and versatile tools for a diverse range of applications. Their capabilities also offer opportunities for business process management, however, these opportunities have not yet been systematically investigated. In this paper, we address this research problem by foregrounding various management tasks of the BPM lifecycle. We investigate six research directions highlighting problems that need to be addressed when using large language models, including usage guidelines for practitioners.

==> sections/background.tex <==
\section{Background}
\label{sec:background}

In this section we give a short introduction into relevant fields for the topic at hand.
This includes \gls{nlp} (\Cref{subsec:natural:language:processing}), \gls{dl} (\Cref{subsec:deep:learning}), and \glspl{llm} (\Cref{subsec:large:language:models}).


\subsection{Natural language processing}
\label{subsec:natural:language:processing}

\acrlong{nlp} as a discipline has its roots at the intersection of linguistics and \gls{ai}, and is part of computer science~\cite{nadkarni2011natural}.
The field is also known as computational linguistics~\cite{9075398} (see~\cite{church2021future} for a historical overview).
It involves various tasks such as text classification, sentiment analysis, machine translation, named entity recognition, reading comprehension, summarization, translation, textual entailment, question answering, semantic similarity assessment, and document classiﬁcation~\cite{radford2019language}.
\gls{nlp} has as a consequence a wide range of applications, from customer service chatbots to medical information extraction from electronic health records. 
The goal of NLP is to build systems that can process, understand, and generate human language, making communication between humans and computers more natural and seamless.

\cite{JMLR:v12:collobert11a}.

In recent years, \gls{nlp} has made remarkable progress with the advent of advanced deep learning models, such as the GPT-3 model, which has demonstrated remarkable performance on various of the above mentioned \gls{nlp} tasks.
These deep learning models are build with building blocks designed to process sequences, such as recurrent neural networks (RNNs) and transformer networks.
When these models are trained on large amounts of text data, often from the internet, they are able to learn the patterns and relationships in language, and as a result extract meaningful information from text data.
With meaningful information we mean a set of useful representations to accomplish a set of tasks.

\cite{hirschberg2015advances}.



\subsection{Deep learning}
\label{subsec:deep:learning}

\paragraph{Machine learning}
\gls{ml} studies algorithms that are \emph{''capable of learning to improve their performance of a task on the basis of
their own previous experience''}~\cite{mjolsness2001machine}. 
Prominent examples of such algorithms are \gls{pca}, decision trees, random forests, and \gls{nn}.
The algorithms developed, and subsequently studied, by \gls{ml} have progressed immensely in the last two decades~\cite{jordan2015machine}.
As of today, they are widely used in academia and commercial products, from computer vision, speech recognition, natural language processing, and robot control~\cite{jordan2015machine}.
One major dimension on how to categorize \gls{ml} algorithms is based on the information that is available in the training data, more specifically, the feedback signal.
On this dimension, \gls{ml} differentiates between the three learning paradigms supervised learning, unsupervised learning, and reinforcement learning.


\paragraph{Supervised learning, Unsupervised learning, and Reinforcement learning}
In supervised learning, the \gls{ml} algorithm receives as an input a collection of pairs, where one pair consists of features representing a concept along with a label.
Importantly, this label is task specific and encodes what the algorithm should learn about the concepts.
Examples of concepts are images and texts.
A given image may be represented by a red, green, and blue feature tensor, or the same image can be represented by a gray scale feature tensor.
Examples for labels are \emph{spam} and \emph{no spam} for a spam classifier, or bounding boxes with annotations (for example the name of a person) for an image.
As is evident from the labels, the key in supervised learning is that we want the algorithm to perform well on a well defined task.
In the \gls{ml} literature this is referred to as task specific.
Using these labels, \gls{ml} differentiates between two types of tasks - on one hand classifications (such as predicting spam or no spam) or regression (such as bounding box regression).
Finally, there are two extreme cases of superpervised learning that are important for \gls{llm} - \emph{few-shot} and \emph{zero-shot} learning.
\emph{Few-shot} learning is when a \gls{ml} algorithm adapts to a new situation with little amount of labelled data, and \emph{zero-shot} learning is when the algorithm can do this with no labelled data at all.
Note here that the definition does not imply any change in the parameters of the model.
For example, you can provide a language model with a few input-output pairs, and the model inverse the mapping function without any parameter changes.


In unsupervised learning, the algorithm only receives a feature tensor of a concept as an input.
And the algorithm then finds structural properties of the concepts present in the feature tensor.
Two big problems this learning paradigm studies are dimensionality reduction and clustering.
In dimensionality reduction, the assumption is that the feature tensor can be reduced to a much lower dimensional representation - and the goal is to find this representation.
Popular methods for this task are \gls{pca} and autoencoders.
In clustering, the assumption is the presence of unknown groups which form a partition (called clusters) in the feature tensor.
The key here is that the clusters are unknown - and hence we can not provide any labels.
Prominent examples of clustering algorithms are k-means and hierarchical clustering.

In reinforcement leaning, the algorithm receives a feature tensor of a concept as an input for which an output is produced, which are then evaluated through rewards.
The algorithm then uses this feedback to improve its future decisions.
This type of learning is used for tasks where the goal is to take actions in an environment to maximize a reward signal.
It is commonly used in robotics, gaming and control systems, among other areas.
The algorithm learns through trial and error, receiving positive or negative rewards for its actions, and adjusts its decision-making process accordingly.
In this paradigm, the algorithm acts as an agent that interacts with its environment and learns how to optimize its behavior based on the rewards it receives.
ChatGPT uses a form of reinforcement learning known as deep reinforcement learning to improve its language generation capabilities - in particular, \emph{''Learning to summarize from human feedback''}~\cite{NEURIPS2020_1f89885d}.
ChatGPT is fine-tuned using a reward signal that assesses the quality of its generated responses, with the goal of maximizing the reward signal over time. The model's ability to learn from the reward signal allows it to generate increasingly relevant and coherent responses.



\paragraph{Deep learning}
\gls{dl} is a \gls{ml} method based on \gls{nn}. 
Specifically, they are \glspl{nn} with many layers stacked on top each other, which enables them to learn multiple layers of representations~\cite{lecun2015deep}.
Importantly, these representations are learned without supervision, which is one key success factor.
Shallow networks, on the other hand, only have a few layers and are therefore not able to learn as complex relationships between inputs and outputs. 
Deep networks are able to handle more complex problems compared to shallow networks, which is why they have become so popular in recent years. 
Combined with the availability of large amounts of data, improvements on how to speed up the optimization, and powerful computing resources, enables them to be trained effectively.
One of the key challenges in deep learning is to avoid overfitting, which is when the network memorizes the training data, instead of learning a general relationship between inputs and outputs. 
This can be prevented through various techniques such as regularization and early stopping.
In the context of natural language processing, deep learning has been particularly effective in tasks such as machine translation, sentiment analysis, and named entity recognition. 
The ability of deep learning to learn multiple layers of representations from input data has proven to be particularly powerful for these tasks. 
This is because natural language processing involves dealing with sequences of words and characters, and the relationships between these sequences are often complex and multi-layered.



\paragraph{Deep learning for natural language processing}
\gls{dl} has proven to be effective in a wide range of \gls{nlp} tasks, including sentiment analysis, text classification, machine translation, and text generation. 
The power of deep learning for \gls{nlp} lies in its ability to automatically learn complex representations of the input data without the need for manual feature engineering. 
The use of large amounts of labeled training data and powerful computational resources has enabled deep learning models to achieve state-of-the-art results in many \gls{nlp} tasks. 
For example, the transformer architecture, introduced in the paper \emph{''Attention is All You Need''} by Vaswani et al.~\cite{vaswani2017attention} has become the standard architecture for many NLP tasks, including language translation and language modeling.


\subsection{Large language models}
\label{subsec:large:language:models}

%
% Add figure showing the growth of number of parameters and training data set size
% https://research.aimultiple.com/gpt/


\paragraph{Large language models}
\gls{llm} are \gls{dl} models that are trained on vast amounts of text data to perform various natural language processing tasks. 
These models, which typically have hundreds of millions or billions of parameters, are designed to capture the complexities and nuances of human language. 
The largest models, such as \gls{gpt}-1 and \gls{gpt}-3, are capable of generating human-like text, answering questions, translating languages, and even coding.
The training process of these models involves processing massive amounts of text data, which is used to learn patterns and relationships between words and phrases. 
These models then use this information to predict the likelihood of a given word or sequence of words, given a context. 
This allows them to generate coherent and contextually relevant text or perform other language-related tasks.
The rise of large language models has resulted in significant advancements in the field of NLP, and they are widely used in various applications, including chatbots, virtual assistants, and text generation systems.

These \gls{llm} are able to perform \emph{few-shot} and \emph{zero-shot} learning with prompt-based learning~\cite{liu2023pre}.


%
% Look up calculation of parameters
%
\paragraph{GPT-1}
In 2018, Radford et al. introduced GPT-1 (also sometimes called simply GPT) with the paper \emph{''Improving language understanding by generative pre-training''}~\footnote{See the \href{https://github.com/openai/finetune-transformer-lm}{GitHub repository of GPT-1} for more information.}~\cite{radford2018improving}.
\gls{gpt}-1 referst to the largest model the authors have trained (110 million parameters).
In the paper, the authors studied the ability of transformer networks trained in two phased for language understanding.
In the first phase, the authors trained a transformer network unsupervised - in particular they trained them to predict the next token given a set of tokens that appeared before (also called unsupervised pre-training, generative pre-training, or in statistics auto-regressive).
In the second phase, the authors fine tuned the transformer networks on tasks with supervised learning (also called discriminative fine-tuning).
In summary, their major finding was that combining task agnostic unsupervised learning in the first phase, and using this model than in a second phase with supervised learning for fine tuning on tasks can lead to performance gains - from 1.5\% on textual entailment to 8.9\% on commonsense reasoning.


\paragraph{GPT-2}
In 2019, Radford et al. introduced GPT-2 with the paper \emph{''Language Models are Unsupervised Multitask Learners''}~\footnote{See the \href{https://github.com/openai/gpt-2}{GitHub repository of GPT-2} for more information.}~\cite{radford2019language}.
Again, \gls{gpt}-2 refers to the largest model they have trained. GPT-2 is hence a scaled up version of GPT-1 in model size (1.5 billion parameters), and also in training data size.
In particular, GPT-2 has roughly more than ten times the number of parameters than GPT-1, and is trained on roughly more than ten times the amount of training data.
They report two major findings.
First, that the unsupervised GPT-2 can outperform language models that are trained on task specific data set, without these data sets being in the training data set of GPT-2.
Second, GPT-2 seems to learn tasks (for example question answering) from unlabeled text data.
In both cases, however, the performance were far from the state-of-the-art.
In summary, their major finding was that \glspl{llm} may be able to learn tasks without the need to train them on these tasks, given that they have sufficient unlabeled training data.


\paragraph{GPT-3}
In 2020, Brown et al. introduced \gls{gpt}-3 with the paper \emph{''Language Models are Few-Shot Learners''}~\footnote{See the \href{https://github.com/openai/gpt-3}{GitHub repository of GPT-3} for more information}~\cite{NEURIPS2020_1457c0d6}.
Unlike the above two cases, \gls{gpt}-3 refers to all the models  the authors have trained - in other words, it refers to a family of models. 
The largest model the authors have trained is \gls{gpt}-3 175B, a model with 175 billion parameters.
In their paper, the authors showed that language models like GPT-3 can learn tasks with only a few examples, hence the title includes \emph{''few-shot learners''}. 
The authors demonstrated this ability by fine-tuning GPT-3 on various tasks, including question answering and language translation, using only a small number of examples.


\paragraph{GPT-4}



\paragraph{ChatGPT}
In 2022, OpenAI introduced a conversational \gls{llm} - called ChatGPT~\cite{ChatGPT}.
As a model, the first version of ChatGPT was based on \gls{gpt}-3.5 and is a sibling to InstructGPT.
\gls{gpt}-3.5 is a \gls{gpt}-3.0 model trained on a training data set that contains text and software code up to the fourth quarter of 2021~\cite{GPT3-5}.
And InstructGPT was introduced in \emph{''Training language models to follow instructions with human feedback ''}~\cite{ouyang2022training}, and is a \gls{gpt}-3 model fine tuned with supervised learning in the first step, and in the second step with reinforcement learning from human feedback~\cite{NEURIPS2020_1f89885d}.
ChatGPT is hence a \gls{gpt}-3.5 model fine tuned for conversational interaction with the user.
In other words, the user interacts with the model via sequence of text (the conversation) to accomplish a task.
For example, we can copy and paste a text into ChatGPTs' input field and ask it to summarize it.
We can even be more specific, we can say that the summary should be 10 sentences long and be written in a preferred style.
Importantly, if we are unhappy with the result we can ask ChatGPT to refine its' own summary without copying and past the text it should summarize again.
At the moment of this writing, ChatGPT can be used with GPT-4.



\paragraph{\acrshort{opt}}
In 2022, Zhang et al. introduced \gls{opt} with the paper \emph{''OPT: Open Pre-trained Transformer Language Models''}
\footnote{See the \href{https://github.com/facebookresearch/metaseq/tree/main/projects/OPT}{GitHub repository of OPT} for more information}~\cite{zhang2022opt}.
The main contribution of this paper is that it shares all artifacts created for this paper - including the nine models - for interested researchers, so the impact of \glspl{llm} can be studied by any researcher.
These models are \gls{gpt}-3 class models in parameter size and performance.


\paragraph{\acrshort{bloom}}
Another open \gls{llm} is \gls{bloom} (176 billion parameters), which was developed in the BigScience Workshop~\cite{scao2022bloom}.


\paragraph{Other large language models}




\subsection{Business process management and large language models}
\label{subsec:business:processes:and:large:language:models}
%
% Write here about promises of large language models.
%

==> sections/related-work.tex <==
\section{Related work}
\label{sec:related:work}

\paragraph{Process modeling, process mining, knowledge graphs, and machine learning}
\cite{10.1007/978-3-031-23515-3_7}


\paragraph{\acrshort{ai} and \acrshort{bpms}}
\cite{dumas2023ai}


\paragraph{\acrshort{nlp} in \acrshort{bpm}}
\cite{van2018challenges}
